Formal Verification of Debates in Argumentation Theory

Humans engage in informal debates on a daily basis. By expressing their opinions and ideas in an argumentative fashion, they are able to gain a deeper understanding of a given problem and in some cases, find the best possible course of actions towards resolving it. In this paper, we develop a methodology to verify debates formalised as abstract argumentation frameworks. We first present a translation from debates to transition systems. Such transition systems can model debates and represent their evolution over time using a finite set of states. We then formalise relevant debate properties using temporal and strategy logics. These formalisations, along with a debate transition system, allow us to verify whether a given debate satisfies certain properties. The verification process can be automated using model checkers. Therefore, we also measure their performance when verifying debates, and use the results to discuss the feasibility of model checking debates.

==> semantics_table.tex <==
\begin{table}
  A set $E \subseteq Args$ of argument is 
  \begin{tabbing}
    %{|c|c|}
%   \hline
 \textbf{Semantics} \ \ \ \= \ \ \ \  \ \ \ \= \textbf{Criteria} \\
 % \hline
 conflict-free \> iff \>
 %it does not attack itself:
 there are no
$a, b \in E$ such that $(a,b) \in Attacks$\\
 admissible \> iff \>  it is conflict free\\
 \> and \>  every argument in $E$ is acceptable w.r.t.~$E$.\\
 %or every argument $b \in Args$ that attacks some $a \in E$, there is some $c \in E$ that attacks $b$ (and defends $a$).\\
 complete \> iff \> it is admissible \\
          \> and \> it contains all arguments that are acceptable w.r.t.~$E$\\
          grounded    \> iff \>  complete\\
          \> and \> minimal w.r.t.~set inclusion \\ 
          preferred   \> iff \>  admissible\\
          \> and \> maximal w.r.t.~set inclusion \\ 
          ideal      \> iff \> admissible\\
          \> and \> a subset of every preferred extension
% \hline
\end{tabbing} 
 \caption{The various extension-based semantics presented in \cite{dung1995acceptability, dung2007computing}.}
\label{tab:semantics}
\end{table}

